GigSense: An LLM-Infused Tool for Workers Collective Intelligence

Collective intelligence among gig workers yields considerable advantages, including improved information exchange, deeper social bonds, and stronger advocacy for better labor conditions. Especially as it enables workers to collaboratively pinpoint shared challenges and devise optimal strategies for addressing these issues. However, enabling collective intelligence remains challenging, as existing tools often overestimate gig workers' available time and uniformity in analytical reasoning. To overcome this, we introduce GigSense, a tool that leverages large language models alongside theories of collective intelligence and sensemaking. GigSense enables gig workers to rapidly understand and address shared challenges effectively, irrespective of their diverse backgrounds. Our user study showed that GigSense users outperformed those using a control interface in problem identification and generated solutions more quickly and of higher quality, with better usability experiences reported. GigSense not only empowers gig workers but also opens up new possibilities for supporting workers more broadly, demonstrating the potential of large language model interfaces to enhance collective intelligence efforts in the evolving workplace.

==> trash.tex <==
https://www.overleaf.com/project/65d525d12d5dc28236845c02

\subsubsection*{\bf  Tools to Support Workers in Collective Action} Over the years different solutions designed to help workers initiate collective action have emerged. For instance,  Catalyst \cite{cheng2014catalyst} was the first attempt at supporting collective action based on ``activation thresholds''. However, while Catalyst is useful for predetermined events, it lacks coordinating features to allow users to coordinate and reach a consensus. This is an important limitation as researchers emphasize the importance of collaboration among workers for the future of gig work, especially in the context of creative tasks \cite{kittur2010crowdsourcing}. A more recent solution that aims to allow workers to collaborate is Turkopticon \cite{irani2013turkopticon} is a browser extension and website designed to enhance transparency and empower workers in the Amazon Mechanical Turk (MTurk) marketplace. Turkopticon allows MTurk workers to review and rate the requesters on the platform. The platform also enables workers to share their experiences, voice concerns, and warn others about potentially problematic requesters. 
Platforms in the form of forums have emerged as well, aiming to foster the sharing of valuable insights and experiences among workers, thereby nurturing a sense of community and collaborative learning. Notably, examples like Turker Nation and Turkerview have arisen in response to the policy adopted by Amazon Mechanical Turk (AMT), where requesters have the discretion to pay only for tasks they deem subjectively satisfactory. However, it's worth noting that Turkopticon, Turker Nation and Turkerview are tailored exclusively for Amazon Mechanical Turk, rendering them inaccessible to gig workers operating on different platforms. 

In this paper we use a more recent initiative as a baseline:  ``We Are Dynamo,'' a forum that was specifically created to facilitate collective action for crowd workers \cite{salehi2015we}.   Through this forum, workers come together, identified common interests, and collaboratively crafted a list of best practices. However, it is important to highlight that ``We Are Dynamo,'' does not facilitate communication, collaboration, and sensemaking. These aspects need to be coordinated outside the platform, which introduces several barriers \cite{johnston2018organizing}. First, the need for external coordination can result in fragmented communication, making it challenging to ensure all relevant parties are engaged in discussions. Second, navigating between platforms can be cumbersome and time-consuming, potentially deterring workers from actively participating. Lastly, the lack of integrated communication tools might inhibit the spontaneous exchange of ideas and hinder the swift organization of collective actions and sensemaking.  Our work builds upon ``We Are Dynamo,' as we incorporate collaborative functionalities, harness the power of AI to enhance idea generation and tailor our system design to facilitate gig workers' sensemaking process to find solutions to their challenges.  

%This paper introduced GigSense, an innovative AI-enhanced system crafted to assist gig workers in comprehending
%and addressing their shared challenges. GigSense facilitates the initial stages of collective intelligence, enabling workers to
%engage in effective sensemaking to collectively propose solutions to their collective problems. Our mixed-method study
%showed that GigSense helped participants to comprehensively understand the collective challenges they face by helping
%them identify more problems, enabling them to propose more viable and diverse solutions more quickly compared to a
%control group. We also found that participants in the GigSense group reported better usability experiences, appreciating
%its role in sensemaking of problems, collaborative solution development, and integrating AI assistance while prioritizing
%human-generated solutions. The positive reception and effective functionality of GigSense underscore its potential to
%transform how gig workers interact with challenges, converting isolated struggles into shared victories. 

%``Gig'' or platform-based work represents one of the most recent labor market trends \cite{watson2021looking}. The popularity of gig work can be attributed to the increased demand for flexibility on the part of employers \cite{mandl2015new}, the desire for greater flexibility on the part of workers \cite{de2016rise} and the fact that it is work facilitated through technology and digital markets, on-demand \cite{johnston2018organizing}.
%Even though gig work can offer economic advantages to socially disadvantaged populations like the unemployed, those in remote areas, and refugees \cite{de2016rise}; it can also have adverse effects on workers, such as unpredictable schedules, fluctuating income, and unreliable long-term employment prospects \cite{peck2012politicizing,de2016rise}.
%Collective action activities (i.e. negotiations, strikes, unionization campaigns)  are ways for workers to advocate for better working conditions \cite{khovanskaya2020bottom}. Gig workers have participated in collective endeavors to enhance their work conditions; however, the results have been mixed.  The reasons vary, from gig platforms not facilitating in-app communication among workers \cite{gray2019ghost} to the geographical dispersal of gig workers \cite{johnston2018organizing}. As they move in and out of short-term "gigs" across different industries \cite{sutherland2017gig}, this inevitably hinders their ability to form a sense of community and identify common interests among themselves \cite{yao2021together}. These characteristics create obstacles for collective organizing efforts, as workers can be challenging to locate, difficult to reach, and hard to engage \cite{yao2021together,webster2016microworkers}. Researchers  acknowledge that participating in collective action increases a worker’s ability to choose better jobs with clear expectations and higher
%remuneration rates \cite{berg2015income}. 
%Even though gig workers have achieved a degree of success in coordinating collaborative efforts to enhance their working conditions \cite{UberSuccess}, systems designed to assist gig workers in organizing collective actions are scarce \cite{johnston2018organizing}. Considering the potential growth in this sector, it becomes crucial to develop solutions that support worker organizing and collective bargaining \cite{johnston2018organizing}. In this paper, we focus on creating a tool to help gig workers in the sensemaking of their challenges and initiating collective action.  

%Our study has limitations: We recruited actual gig workers as participants who have diverse skills and come from diverse geographical backgrounds \cite{berg2021working}, which introduces potential individual differences that could impact generalizability. To mitigate these differences, we established inclusion criteria, requiring participants to have a minimum of one year of gig platform experience. This ensured they possessed an understanding of the challenges in gig work, enabling meaningful engagement and evaluation of our system. \blu{Our study also had a relatively small sample size of participants. However, this sample size aligns with HCI's mixed methods approach prioritizing qualitative depth over quantitative breadth \cite{yen2020decipher,clark2015mixed,george2021mixed}. Through our user studies and exit interviews, we gathered extensive data from each participant. This facilitated an integrated analysis of diverse data types to produce actionable insights on utilizing LLMs to assist worker sensemaking and collective action. While the sample size may limit the generalizability of our study, it enabled a rich, focused understanding of gig workers' interactions and experiences. As future work validates findings across broader and more large-scale samples and various age groups, our rigorous analysis nonetheless provides valuable in-depth insights on LLMs' potential to enhance worker discourse and collaboration around shared challenges.} Furthermore, we integrated real-world complaint data about gig platforms and actual conversations of gig workers to contextualize the challenges faced by gig workers more broadly than what our specific participants experienced. It may also not be feasible to address all gig worker challenges, even with the help of systems like GigSense. Future research could categorize these issues into those with and without clear solutions. It could explore the potential of using LLMs and interactive interfaces to improve problem-solving, particularly for complex issues. A longitudinal study with prolonged participant interaction could have offered more behavioral data on social interactions facilitated by our system. However, due to the limited support for gig worker collective action, our system and study remain significant. Upon publication, we will open-source our platform, allowing the scientific community to conduct longitudinal studies on intelligent systems for collective action, potentially benefiting other actors in their collective endeavors. We also acknowledge large language models (LLMs) can generate erroneous solutions which can lead to unintended consequences. To address this, our system prioritizes human-generated solutions over AI suggestions. We also incorporated a disclaimer warning users of potential bias and error. The LLM responses serve merely as hints to guide workers, who remain the final decision-makers. \blu{However, it is important to acknowledge that introducing the LLM on this new platform, could convey a message to users, suggesting: ``We can address any of your queries." This could mislead users into perceiving the platform as an all-encompassing solution for information retrieval. Future studies should explore how disclaimers might better inform gig workers about the LLM's limitations. Note also that our focus was on examining how LLMs combined with interactive interfaces enhance solution creation compared to traditional interfaces, as our goal was to understand the impact of these advanced human-computer interactions (HCI). Future research could investigate the standalone effectiveness of LLMs in supporting workers and the specific benefits that interactive interfaces add. Prior studies suggest that the integration of LLMs with interactive interfaces will likely yield superior outcomes \cite{huang2023causalmapper,jiang2023graphologue,girotra2023ideas,yuan2022wordcraft}, especially as not everyone is an expert in prompting the LLMs \cite{Challangestoprompt}}.

%Prior work on creativity support tools demonstrates how a computational semantic model of a solution space can enable interventions that substantially improve the number, quality and diversity of ideas.

\subsubsection*{\bf \blu{Interpreting Crowdsourced Contributions}.} \blu{To assess how gig workers' contributions differ using our tool versus a control interface, we took inspiration from prior research studying crowds' contributions to varying interfaces \cite{yen2020decipher,siangliulue2016ideahound,jasim2021communityclick,jasim2021communitypulse}. For example, Yen et al. \cite{yen2020decipher},  introduced a unique crowdsourcing tool for helping crowds to visualize and organize design feedback by topic and sentiment. The paper employed a mixed methods study, including a between-subjects study with 20 participants and interviews, to evaluate its new system for design. We also decided to adopt a between-subjects study and interviews to assess workers' interactions with our system against a baseline, recruiting also comparable number of participants. Siangliulue et al.'s paper \cite{siangliulue2016ideahound} also influenced our approach to studying crowd contributions. Their study included a between-subject analysis of crowd behavior for assessing crowd-generated outcomes, specifically measuring idea quantity, diversity, and creativity compared to a control group. Drawing inspiration from this research, we evaluated gig workers' interactions with our system to study the number of problems identified, the number of solutions proposed, and the diversity of proposed solutions. This allowed us to compare our system against a control setup. Other research that influenced us is that from Mahmood et al. \cite{jasim2021communityclick,jasim2021communitypulse}. These papers centered on creating systems for community feedback and analysis. The paper used interviews and crowd behavior studies to evaluate the effectiveness of their proposed systems. Inspired by this, we also integrate interviews and interaction activity analysis to understand gig workers' perspectives on our system and its effectiveness.}

discusss'

%Employing LLMs demands substantial computational resources, leading to energy-intensive processes \cite{hoffmann2022training}. For instance, the training of GPT-3  with 175B parameter consumed considerable compute during pre-training \cite{li2023survey}, far exceeding the needs of a 1.5B parameter GPT-2 model \cite{zhang2023instruction,biderman2023pythia}. This necessitates a thorough evaluation of cost and efficiency when integrating LLMs into the human-centered AI interfaces we design \cite{finn2016connection,bender2021dangers}. It is crucial to assess the resources needed for training LLMs and the distribution of such resources across the model's lifecycle, as well as assessing the amount of computation that is needed for fine-tuning the LLMs models if needed \cite{naser2023we}. However, it is important to recognize that despite the significant training costs, large pre-trained models like GPT-3 have been demonstrated to be highly efficient post-training \cite{liang2022holistic}. Furthermore, techniques like ```model distillation'' can further economize the costs \cite{liang2020mixkd,dasgupta2023cost}. Notice that model distillation, in the context of LLMs, involves transferring knowledge and information from a larger, complex LLM to a smaller, more efficient model \cite{zhao2019extreme}. This empowers the smaller model to execute tasks with fewer computational resources and memory while still capitalizing on the expertise embedded within the larger model. Given the advancements in image recognition and neural networks, we expect that algorithmic progress will improve LLM efficiency over time \cite{liu2019recent,hernandez2020measuring}. It is also important to acknowledge that while LLMs excel in generating solutions and summarizing problems, they are not exempt from limitations. The solutions and summaries that LLMs generate stem from learned patterns within existing data, potentially perpetuating biases or flawed assumptions present in their training data \cite{ferrara2023should,kirk2021bias,rozado2023political}. Recent research underscores the need for active intervention to address biases in LLMs \cite{thakur2023language,chen2021evaluating}. Just identification of the biases is not sufficient. Substantial work remains, particularly in effectively communicating potential biases \cite{hamborg2022frame}. We advocate for a holistic approach to bias mitigation rather than a singular focus on metric-based ``elimination," as this approach has inherent limitations \cite{dhamala2021bold,liu2021mitigating}. Future endeavors could explore transparent interfaces communicating biases to stakeholders, aiding in informed decision-making and ultimately enhancing users' success in integrating LLMs into their workflows \cite{piktus2023roots,liao2023ai}. \blu{Note however, that while GigSense may warn users about potential LLM errors (e.g., hallucinations), the implications of providing plausible but incorrect solutions are not fully understood. In GigSense's current design, workers are considered the final decision-makers and are responsible for implementing the solutions. Future research could investigate various human-AI collaboration models and responsibility frameworks to determine the most effective approach in this context \cite{kulkarni2023llms}}.

\subsusection{}

%Collective intelligence among gig workers holds promise for increased information exchange, builds social bonds, and acts as a catalyst for advocating better labor conditions, Nevertheless, despite efforts from researchers, practitioners, and workers themselves to design tools to support collective intelligence among gig workers, enabling collective intelligence continues to present challenges. Existing tools often assume that gig workers have ample time and equal skills for problem analysis and solution proposals, which is often not the case. To address this, we introduce GigSense, a tool integrating large language models with collective intelligence and sensemaking theories. It assists gig workers to swiftly comprehend collective challenges and devise effective solutions, regardless of their backgrounds. In a between-subject mixed method user study, GigSense users demonstrated improved performance over those using a state-of-the-art control interface, identifying more problems, and producing faster and higher-quality solutions. They also reported enhanced usability experiences. GigSense opens new design possibilities for empowering not only gig workers but also knowledge workers more broadly, showcasing how interfaces with large language models can support collective intelligence efforts critical to the future of work.


\blu{In this paper, we present two key contributions: (1) a system that combines LLM with an interactive interface to aid gig workers in problem-solving, fostering the initiation of collective action; and (2) a between-subjects study demonstrating that GigSense not only accelerates the problem-solving process, but also enhances the feasibility and diversity of solutions generated by workers. We conclude by discussing the impacts of LLMs on sensemaking and workers, and suggest future research paths in this area.}


%\blu{Our mixed-method between-subjects study revealed that GigSense supported workers' sensemaking process, speeding it up, and aided gig workers in identifying more problems, as well as proposing more feasible and more diverse solutions.} \blu{GigSense is an important step towards promoting collective intelligence among gig workers and addressing their distinct needs. Gig workers, who often face unique and scattered challenges, usually work in solitude without a common platform for easily identifying their problems and generating solutions \cite{10.1145/3533406.3533424,yao2021together}. GigSense fills this gap by providing a shared platform where gig workers can unite to comprehend their challenges and devise tangible solutions. Drawing on research that shows shared digital resources can promote community building \cite{sawyer2014digital,barley1986technology}, GigSense stands out as a potential key resource for an often fragmented workforce \cite{10.1145/3533406.3533424,yao2021together}. It has the potential to serve not just as a tool for organization, but also as a catalyst for creating gig worker communities that collaborate and support each other in collective endeavors \cite{yao2021together,lehdonvirta2022cloud}. We also expect that GigSense will further empower gig workers by revealing systemic issues through its interactive interfaces and aggregated data. Its AI-enhanced interface could help to highlight recurring client problems, contract disputes, and payment delays, encouraging workers to view these as collective, not isolated, problems. Recognizing these shared challenges can foster group identity and solidarity, essential for collective intelligence. \cite{tajfel1979integrative,cohen2003collective,van2008toward,tajfel2004social}. Additionally, we expect that GigSense's intelligent interface will not only help to raise awareness, but will also assist workers in developing better strategies and solutions for negotiation, potentially improving contract conditions, or enhancing communication and advocacy.}



leveraging online communities and social media, has significantly improved labor conditions on platforms like Upwork, Amazon Mechanical Turk, and Uber. Through organizing efforts, such as strikes, gig workers have achieved higher wages and better treatment. Notably, in some cities, they've successfully negotiated improved working conditions and better regulations, demonstrating the effectiveness of collective intelligence in implementing pro-worker policies and facilitating collective bargaining with gig platforms.


\blu{It is important to recognize that parts of our design are centered on facilitating workers' rapid sensemaking, thereby supporting the initial stages of collective intelligence \cite{zhang2014wedo,shaw2014computer}. This might appear to challenge the conventional, lengthy nature of sensemaking \cite{weick1995sensemaking,dervin2001sense}. Our goal is to understand how blending interactive interfaces with LLMs could potentially maintain the depth and quality of sensemaking processes while simultaneously enhancing their speed and efficiency. It is also key to recognize that the effectiveness of sophisticated intelligent interfaces, such as GigSense, is not immediately apparent; these may be more complex than simple list-based methods, potentially leading to cognitive overload and lower quality outputs \cite{sweller1994cognitive,norman2013design}. We aim to deepen our understanding of these dynamics to introduce innovative systems that facilitate broader participation in the sensemaking process to initiate collective intelligence.}


To initiate collective intelligence among gig workers, we introduce GigSense—a novel platform designed to \blu{help in sensemaking for} collaborative problem-solving within the gig worker community. Leveraging Sense-Making Theory \cite{pirolli2005sensemaking} and the inherent capabilities of large-language models (LLMs) in text generation and processing, we implement an LLM-enhanced interactive \blu{sensemaking} interface within GigSense. This synergy empowers gig workers to meticulously dissect their challenges and potential solutions, examining them from diverse dimensions and viewpoints. The GigSense platform also empowers gig workers to zoom in for detailed scrutiny or zoom out for a panoramic understanding of their problems. This sets it apart from existing technologies \cite{salehi2015we}, which mainly present workers with an extensive list of problems and solutions, lacking mechanisms for exploring different facets of the problems or achieving a comprehensive understanding of workplace dynamics and crucial matters. \blu{GigSense also utilizes LLMs to assist workers in collectively brainstorming solutions to their problems.} 

%However, despite the occasional success stories, gig worker collective intelligence is rare \cite{globalanalysisofdigitalworkprotest}. As a result, most gig workers' problems remain unresolved. \blu{We contend that a key challenge for gig worker collective intelligence} stems from the scarcity of available technologies designed to assist gig workers in collective problem-solving \cite{johnston2020labour,shaw2014computer,zhang2014wedo,gray2019ghost,lehdonvirta2022cloud}.  For example, technologies like Dynamo or Coworker.org allow workers to share their problems, upvote the most crucial ones, as well as propose and upvote solutions to those problems \cite{salehi2015we,demaria2016future}. These technologies typically employ list-based interfaces to present the problems and solutions, and the lists are usually sorted based on the upvotes. However, list-based interfaces can restrict the exploration of problems and solutions from various perspectives, impeding a deep dive into their complexities, as well as obtaining a grasp of the entire problem-solution landscape \cite{li2023dimensions,10.1145/3359310,10.1145/3533406.3533424,mattsson2015sense,sentido,weick1995sensemaking}. This limitation can hinder gig workers' ability to effectively prioritize critical issues like identify optimal solutions \cite{wood2019platform}. The absence of interfaces that facilitate comprehensive problem-solving analysis can lead to workers focusing on trivial problems or irrelevant solutions, ultimately hindering workers' potential to drive meaningful change \cite{CIBook}. \blu{Note that this challenge relates to the early phases of collective action, involving understanding shared issues and developing solutions to address them \cite{boomorbane}.}





%Gig workers, especially digital \blu{knowledge gig worker}s, face distinct communication skill demands \cite{wood2023dynamics}. These demands include unpaid transactional communication tasks like composing cover letters, engaging in client conversations, addressing client queries, emphasizing strengths, and negotiating deadlines and rates \cite{jarrahi2019algorithmic,gray2019ghost,toxtli2021quantifying}. These tasks are both time-consuming and unpaid, often prompting \blu{gig knowledge workers} to prefer repeat clients to reduce these interactions \cite{hulikal2022collaboration}. It is also important to note that these unpaid transactional costs can be even more challenging for gig workers who are non-native English speakers or have difficulty articulating their ideas\cite{panaligan2022we,kowalik2022job,thompson2019digital}.

%One key category of \blu{text based generative AI} tools for \blu{gig knowledge workers} should focus on enhancing communication, as also emphasized by participants in our study. While existing tools like ChatGPT can already aid in various communication tasks, \blu{gig knowledge workers} may not be fully aware of their potential use for such purposes or the most effective prompts to employ \cite{white2023prompt,wang2023review}. Our results highlight this point, as few workers used existing commercial tools for communication improvement. Even those who did still desired tools tailored to \blu{knowledge gig worker} communication needs. This emphasizes the importance of specialized, task-specific tools for enhancing \blu{knowledge gig worker} communications. One design area to explore is thus creating specialized tools for enhancing \blu{knowledge gig worker} communications in virtual meetings. Gig Knowledge work frequently involves online interactions \cite{blyth2022self}, and many platforms offer virtual meeting and video call support. A substantial body of research is emerging in the realm of enhancing virtual meetings \cite{10.1145/3411764.3445615}, including intelligent tool design to promote inclusivity and investigations into the challenges of crafting suitable meeting technologies \cite{saatcci2019hybrid}. Considering our findings, there is potential in creating \blu{text based generative AI} tools tailored for virtual meetings to support workers. These tools could offer assistance in various aspects, such as outlining discussion points with clients, providing conversation starters, or even suggesting ways to enhance their virtual backgrounds for a more professional appearance \cite{joowon2021enhancing}. Aligning these tools with existing research on virtual meetings could yield valuable resources for \blu{gig knowledge workers} \cite{bleakley2022bridging,gonzalez2022making,margariti2022automated}.

%It is also important to consider that introducing generative AI tools for gig worker communication may inadvertently create an unfair environment and set unreasonable expectations for non-native English speakers. Clients or requesters may start expecting all workers to communicate fluently in English, which could result in workers being overlooked for jobs even if they possess the necessary skills. To address this, it is important to draw insights from research on equitable tool distribution \cite{kraemer2009one,angel2015participatory}, ensuring that these generative AI tools are made available to all workers, preventing the exacerbation of inequalities \cite{williams2019perpetual}. Additionally, exploring open-source and open access tool distribution could help mitigate socioeconomic disparities among gig workers arising from uneven access to new technologies \cite{lerner2005economics,nicoletti2023disadvantaged}.


%Our design of Office-Mind AI and our usability study showcased the value that AI tools that act as personal, independent managers and secretaries could bring to gig workers.  We recommend designing AI tools that can take on traditional office roles to support gig workers, but  without imposing penalties or surveillance (i.e., the tools should focus on the well-being of the workers instead of focusing on how to increase the profits for the gig platforms. )  Future research should explore how AI can take on these traditiuonal roles while enhancing workplace structure and well-being, including integrating health activities and phishing protection, to better support gig knowledge workers.

%The absence of conventional organizational support constitutes a significant source of uncertainty in gig work \cite{bryant2020liquid,caza2022working,callanan2017career}. However, workers' interactions with their personal ecosystem enable them to not only thrive amid this uncertainty, but also effectively manage its associated stresses \cite{jarrahi2021flexible}. How workers compensate for the lack of traditional organizational support and protections has been studied in recent research \cite{dunn2023dynamics,de2022understanding,jiang2023more,lascau2023time}. For example,  Petriglieri et al. \cite{petriglieri2019agony} highlighted that freelance workers establish their own "personal holding environments." These environments encompass a network of psychological connections involving personal routines, relationships, physical spaces, and a sense of purpose. They serve as a means for gig workers to emulate the advantages typically offered by traditional workplaces which have much more structure \cite{duggan2020algorithmic,mohlmann2021algorithmic}. In this context, our findings illustrate that \blu{gig knowledge workers}' perceptions of AI tools \blu{, in the form of text based generative ais,} encompass roles typically associated with traditional workplaces. This not only emphasizes Petriglieri et al \cite{petriglieri2019agony}'s  insights but also unveils new dimensions of future work. More precisely, future work could investigate how generative AI tools could seamlessly fit into these personal holding environments, potentially reintroducing elements of structure into the dynamic world of gig work. Our current findings also indicate that gig workers are actively seeking AI tools capable of taking on managerial and secretarial responsibilities, roles commonly encountered in structured and conventional work environments \cite{wichroski1994secretary}. 

%We recommend designing AI tools that assist gig workers in structuring their daily work effectively. Some workers may benefit from having a manager-like tool to organize their work and meet deadlines. However, it is worth noting that intriguingly, none of our participants envisioned this AI manager as an integral component of the digital labor platform. Instead, they preferred a personal AI manager that was independent of the gig platform, and that they could control, enabling them to follow its guidance or deactivate it as needed. \blu{gig knowledge workers} also did not anticipate a manager tool that penalizes them; they desired a supportive tool without constant surveillance or potential devaluation for missing deadlines \cite{duke202224,ball2010workplace}. Therefore, we advocate for AI structuring tools to be independent of the digital labor platform, granting workers the freedom to decide how closely they want to follow the tool's recommendations.

%Our \blu{design activities} also unveiled an important insight: workers envisioned these AI tools assuming human-like roles, effectively carrying out tasks typically associated with human agents (e.g., secretaries or managers). Rather than envisioning a mere task-delivery tool, \blu{gig knowledge workers} imagined intelligent agents capable of performing these tasks. Tools emulating human roles could alleviate workers' cognitive load by embodying familiar roles \cite{hackel2023social}, sparing workers the mental effort required to understand how the tool operates and what tasks to delegate to it \cite{waldrop2022invisible,wahn2023offloading}. Furthermore, these tools can introduce consistency into gig workers' lives \cite{cheon2012effects}, allowing them to concentrate on execution without the need to decipher their functionality, as these roles are already familiar and understood \cite{wahn2023offloading}. Thus, we recommend to present \blu{text based generative AI} tools as agents that mimic\blu{, and specialize in,} human roles.

%This direction also encourages exploration into worker well-being. 
%As replicating organizational support can contribute to a sense of security among workers \cite{rhoades2002perceived,eriksson2009social}, and considering that uncertainty within gig knowledge work can be a significant source of psychological stress \cite{pathak2012role}, it follows that introducing more structure into the workplace could potentially enhance worker well-being. 
%Therefore, we propose investigating worker well-being as another dimension for examining the impact of AI in personal holding environments. 
%We recommend exploring the design of \blu{text based generative AI} tools that not only enhance the structural aspects of gig workers' workplaces but also contribute to improving their well-being.
%Possible connections can also include research on integrating physical and mental health activities in the workplace such as step counting \cite{10.1145/1930488.1930510} and meditation \cite{10.1145/3025453.3025914,kitson2018immersive}, which have been proven to increase worker well being, and adapting these considerations for the gig knowledge worker.
%Additionally, improving protections against phishing can improve worker security, and recent research has shown new techniques for dealing with such attacks \cite{10235951}---integrating defensive measures into the gig knowledge work place can also improve a workers environment.


Through our interviews, design activities, and deep engagement with research, we've identified key directions for creating text-based generative AI tools for gig knowledge workers, detailed in subsequent sections. Specifically, we focus on: (1) Designing AI tools for workplace structure; (2) Enhancing worker communication strategies; and (3) Integrating data analytics for improved decision making.

%\blu{Through our interviews, interactive design activities, and by engaging deeply with existing research \cite{zhang2022algorithmic,zhang2023stakeholder,blyth2022self}, we have identified several promising future directions for designing text-based generative AI tools for gig knowledge workers. These are discussed in detail in the following sections.} \blu{In particular, there are three areas of future directions which we discuss: (1) Designing text-based Generative AI tools for workplace structure; (2) Using text-based Generative AI to improve worker communication strategies; and (3) Applying data analytic alongside text-based generative AI tools for superior worker decision making.} 




%https://libros.metabiblioteca.org/server/api/core/bitstreams/d8bc08aa-c0c8-420b-9d20-95c0ffefe6b3/content

%This module serves as a virtual personal secretary for gig workers. It combines an interactive dashboard with generative AI to empower gig workers to collaborate with AI and streamline administrative tasks, including email drafting, advanced grammar checks, language translation services, and preparation of NDAs. Through the interactive interface, workers share their knowledge about the type of emails, translations, gramnmaer checks, and NDAs they need, and the generative AI shares its rich knowledge to draft professional documents for each of the rubrics that workers desire. Workers can then utilize the chat based interface to iterate and improve the documents based on their knowledge, and through this create a strong human-AI collaborations for preparing strong documents for their jobs. 

What sets OfficeMind AI apart is its integration with collective intelligence, learning from user interactions and feedback to improve and personalize assistance. It combines generative AI with a feedback loop from its user base to refine its algorithms, ensuring relevance and efficacy for gig workers. OfficeMind AI is designed to evolve with its users, simplifying tasks and allowing them to focus on their core work.


Acting as both a personal secretary and a strategic manager, OfficeMind AI is dedicated to optimizing the efficiency and productivity of gig workers, providing them with a comprehensive support system designed to elevate their work experience and outcomes.

%Guided by our design goals, we created OfficeMind AI, an online system equipped with state-of-the-art generative AI and a dashboard, designed to facilitate AI collaborations with gig knowledge workers, especially to support them in tasks they could not easily do on their own or with their current institutional support (i.e., support from the paltforms themselves). For this purpose, Office Mind AI functions as both a personal secretary and manager for workers.



module extends the concept of collective intelligence by assisting users in crafting professional profiles that are informed by the successes and feedback of a wide network of peers. It analyzes effective profiles, cover letters, and bios across various platforms and industries, applying these insights to help users present themselves in the best possible light. This process not only individualizes branding efforts but does so by drawing upon the collective efficacy of strategies proven to resonate within the gig economy.

Additionally, the module could enhance its connection to collective intelligence theories by incorporating a feedback loop where users can rate the effectiveness of their personalized schedules and branding strategies. This feature would allow the system to refine its algorithms further based on user satisfaction and outcomes, embodying a self-improving system that becomes more attuned to the needs and preferences of gig workers over time.

Moreover, by facilitating a community platform within the module, gig workers could share tips, advice, and experiences, further enriching the collective data pool from which the AI learns. This feature would not only foster a sense of community among users but also enhance the module's capabilities through a more dynamic and diverse dataset, driving innovation and personalization to new heights.

%In summary, OfficeMind AI's module embodies principles of collective intelligence by leveraging aggregate data and user feedback to continuously improve its personal management services for gig workers. This approach not only enhances individual productivity and marketability but also contributes to a more adaptable and intelligent system capable of meeting the evolving needs of the gig economy.


This approach addresses the gap in gig work by providing support in scheduling tasks, leveraging both the worker's insights and AI capabilities. Through this, the module fills the role of the manager (missing from gig work) who can guide workers on how to effectively manage their time to meet their client deadlines and manage their desired work schedules. 


analyze patterns and feedback from a broad spectrum of gig workers. This approach allows it to adapt and evolve scheduling algorithms based on collective behavior and success rates, essentially learning from the aggregated data to optimize individual schedules. This feature mirrors the essence of collective intelligence by synthesizing diverse individual inputs into a coherent, optimized scheduling strategy that benefits each user uniquely.


the collective insights and data from a vast number of gig workers' experiences, preferences, and outcomes to continually refine and personalize its offerings.


through its use of generative AI for both time management and personal branding. Collective intelligence emerges when individual efforts and knowledge are aggregated and coordinated, often through technology, to create a smarter, more capable system. In this context, the module leverages the collective insights and data from a vast number of gig workers' experiences, preferences, and outcomes to continually refine and personalize its offerings.

